Explaining How Deep Neural Networks Forget by Deep Visualization

Explaining the behaviors of deep neural networks, usually considered as black boxes, is critical especially when they are now being adopted over diverse aspects of human life. Taking the advantages of interpretable machine learning (interpretable ML), this paper proposes a novel tool called Catastrophic Forgetting Dissector (or CFD) to explain catastrophic forgetting in continual learning settings. We also introduce a new method called Critical Freezing based on the observations of our tool. Experiments on ResNet articulate how catastrophic forgetting happens, particularly showing which components of this famous network are forgetting. Our new continual learning algorithm defeats various recent techniques by a significant margin, proving the capability of the investigation. Critical freezing not only attacks catastrophic forgetting but also exposes explainability.

==> samplepaper <==
\begin{thebibliography}{10}
\providecommand{\url}[1]{\texttt{#1}}
\providecommand{\urlprefix}{URL }
\providecommand{\doi}[1]{https://doi.org/#1}

\bibitem{che2016interpretable}
Che, Z., Purushotham, S., Khemani, R., Liu, Y.: Interpretable deep models for
  icu outcome prediction. In: AMIA Annual Symposium Proceedings. vol.~2016,
  p.~371. American Medical Informatics Association (2016)

\bibitem{dabkowski2017real}
Dabkowski, P., Gal, Y.: Real time image saliency for black box classifiers. In:
  Advances in Neural Information Processing Systems. pp. 6967--6976 (2017)

\bibitem{goodfellow2013empirical}
Goodfellow, I.J., Mirza, M., Xiao, D., Courville, A., Bengio, Y.: An empirical
  investigation of catastrophic forgetting in gradient-based neural networks.
  arXiv preprint arXiv:1312.6211  (2013)

\bibitem{hou2018lifelong}
Hou, S., Pan, X., Change~Loy, C., Wang, Z., Lin, D.: Lifelong learning via
  progressive distillation and retrospection. In: Proceedings of the European
  Conference on Computer Vision (ECCV). pp. 437--452 (2018)

\bibitem{kemker2018measuring}
Kemker, R., McClure, M., Abitino, A., Hayes, T.L., Kanan, C.: Measuring
  catastrophic forgetting in neural networks. In: Thirty-second AAAI conference
  on artificial intelligence (2018)

\bibitem{kirkpatrick2017overcoming}
Kirkpatrick, J., Pascanu, R., Rabinowitz, N., Veness, J., Desjardins, G., Rusu,
  A.A., Milan, K., Quan, J., Ramalho, T., Grabska-Barwinska, A., et~al.:
  Overcoming catastrophic forgetting in neural networks. Proceedings of the
  national academy of sciences  \textbf{114}(13),  3521--3526 (2017)

\bibitem{li2017learning}
Li, Z., Hoiem, D.: Learning without forgetting. IEEE transactions on pattern
  analysis and machine intelligence  \textbf{40}(12),  2935--2947 (2017)

\bibitem{lin2014microsoft}
Lin, T.Y., Maire, M., Belongie, S., Hays, J., Perona, P., Ramanan, D.,
  Doll{\'a}r, P., Zitnick, C.L.: Microsoft coco: Common objects in context. In:
  European conference on computer vision. pp. 740--755. Springer (2014)

\bibitem{ling2019unified}
Ling, C.X., Bohn, T.: A unified framework for lifelong learning in deep neural
  networks. arXiv preprint arXiv:1911.09704  (2019)

\bibitem{michieli2019incremental}
Michieli, U., Zanuttigh, P.: Incremental learning techniques for semantic
  segmentation. In: Proceedings of the IEEE International Conference on
  Computer Vision Workshops. pp.~0--0 (2019)

\bibitem{nguyen2019toward}
Nguyen, C.V., Achille, A., Lam, M., Hassner, T., Mahadevan, V., Soatto, S.:
  Toward understanding catastrophic forgetting in continual learning. arXiv
  preprint arXiv:1908.01091  (2019)

\bibitem{nguyen2019contcap}
Nguyen, G., Jun, T.J., Tran, T., Kim, D.: Contcap: A comprehensive framework
  for continual image captioning. arXiv preprint arXiv:1909.08745  (2019)

\bibitem{shmelkov2017incremental}
Shmelkov, K., Schmid, C., Alahari, K.: Incremental learning of object detectors
  without catastrophic forgetting. In: Proceedings of the IEEE International
  Conference on Computer Vision. pp. 3400--3409 (2017)

\bibitem{simonyan2013deep}
Simonyan, K., Vedaldi, A., Zisserman, A.: Deep inside convolutional networks:
  Visualising image classification models and saliency maps. arXiv preprint
  arXiv:1312.6034  (2013)

\bibitem{tasar2019incremental}
Tasar, O., Tarabalka, Y., Alliez, P.: Incremental learning for semantic
  segmentation of large-scale remote sensing data. IEEE Journal of Selected
  Topics in Applied Earth Observations and Remote Sensing  \textbf{12}(9),
  3524--3537 (2019)

\bibitem{tran2021simple}
Tran, T.Q., Nguyen, G.V., Kim, D.: Simple multi-resolution representation
  learning for human pose estimation. In: 2020 25th International Conference on
  Pattern Recognition (ICPR). pp. 511--518. IEEE (2021)

\bibitem{yosinski2015understanding}
Yosinski, J., Clune, J., Nguyen, A., Fuchs, T., Lipson, H.: Understanding
  neural networks through deep visualization. arXiv preprint arXiv:1506.06579
  (2015)

\bibitem{zeiler2014visualizing}
Zeiler, M.D., Fergus, R.: Visualizing and understanding convolutional networks.
  In: European conference on computer vision. pp. 818--833. Springer (2014)

\bibitem{zenke2017continual}
Zenke, F., Poole, B., Ganguli, S.: Continual learning through synaptic
  intelligence. In: Proceedings of the 34th International Conference on Machine
  Learning-Volume 70. pp. 3987--3995. JMLR. org (2017)

\bibitem{zhai2019lifelong}
Zhai, M., Chen, L., Tung, F., He, J., Nawhal, M., Mori, G.: Lifelong gan:
  Continual learning for conditional image generation. In: Proceedings of the
  IEEE International Conference on Computer Vision. pp. 2759--2768 (2019)

\bibitem{zintgraf2017visualizing}
Zintgraf, L.M., Cohen, T.S., Adel, T., Welling, M.: Visualizing deep neural
  network decisions: Prediction difference analysis. arXiv preprint
  arXiv:1702.04595  (2017)

\end{thebibliography}

